Arrival Directions of Cosmic Rays above 32 EeV from Phase One of the Pierre Auger Observatory

A promising energy range to look for angular correlation between cosmic rays of extragalactic origin and their sources is at the highest energies, above few tens of EeV ($1\:{\rm EeV}\equiv 10^{18}\:$eV). Despite the flux of these particles being extremely low, the area of ${\sim}\:3{,}000 \: \text{km}^2$ covered at the Pierre Auger Observatory, and the 17-year data-taking period of the Phase 1 of its operations, have enabled us to measure the arrival directions of more than 2,600 ultra-high energy cosmic rays above $32\:\text{EeV}$. We publish this data set, the largest available at such energies from an integrated exposure of $122{,}000 \: \text{km}^2\:\text{sr}\:\text{yr}$, and search it for anisotropies over the $3.4\pi$ steradians covered with the Observatory. Evidence for a deviation in excess of isotropy at intermediate angular scale, with ${\sim}\:15^\circ$ Gaussian spread or ${\sim}\:25^\circ$ top-hat radius, is obtained at the $4\:\sigma$ significance level for cosmic-ray energies above ${\sim}\:40\:\text{EeV}$.

==> aastex_authorlist.tex <==
% created on 2022-04-04
\author{P.~Abreu}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Aglietta}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{J.M.~Albury}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{I.~Allekotte}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{K.~Almeida Cheminant}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Almela}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{J.~Alvarez-Mu\~niz}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{R.~Alves Batista}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{J.~Ammerman Yebra}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{G.A.~Anastasi}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{L.~Anchordoqui}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{B.~Andrada}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{S.~Andringa}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{C.~Aramo}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{P.R.~Ara\'ujo Ferreira}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{E.~Arnone}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{J.~C.~Arteaga Vel\'azquez}
\affiliation{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, Michoac\'an, M\'exico}

\author{H.~Asorey}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Assis}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{G.~Avila}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{E.~Avocone}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{A.M.~Badescu}
\affiliation{University Politehnica of Bucharest, Bucharest, Romania}

\author{A.~Bakalova}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~Balaceanu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{F.~Barbato}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.A.~Bellido}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}
\affiliation{Universidad Nacional de San Agustin de Arequipa, Facultad de Ciencias Naturales y Formales, Arequipa, Peru}

\author{C.~Berat}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{M.E.~Bertaina}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{G.~Bhatta}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{P.L.~Biermann}
\altaffiliation{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}

\author{V.~Binet}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{K.~Bismark}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{T.~Bister}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{J.~Biteau}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}

\author{J.~Blazek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Bleve}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{J.~Bl\"umer}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Boh\'a\v{c}ov\'a}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{D.~Boncioli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{C.~Bonifazi}
\affiliation{International Center of Advanced Studies and Instituto de Ciencias F\'\i{}sicas, ECyT-UNSAM and CONICET, Campus Miguelete -- San Mart\'\i{}n, Buenos Aires, Argentina}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{L.~Bonneau Arbeletche}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{N.~Borodai}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.M.~Botti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Brack}
\altaffiliation{Colorado State University, Fort Collins, CO, USA}

\author{T.~Bretz}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{P.G.~Brichetto Orchera}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{F.L.~Briechle}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{P.~Buchholz}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{A.~Bueno}
\affiliation{Universidad de Granada and C.A.F.P.E., Granada, Spain}

\author{S.~Buitink}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{M.~Buscemi}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{M.~B\"usken}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{K.S.~Caballero-Mora}
\affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}

\author{L.~Caccianiga}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{F.~Canfora}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{I.~Caracas}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{R.~Caruso}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{A.~Castellina}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{F.~Catalani}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{G.~Cataldi}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.~Cazon}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{M.~Cerda}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{J.A.~Chinellato}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{J.~Chudoba}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Chytka}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{R.W.~Clay}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.C.~Cobos Cerutti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{R.~Colalillo}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{A.~Coleman}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}

\author{M.R.~Coluccia}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{R.~Concei\c{c}\~ao}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{A.~Condorelli}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{G.~Consolati}
\affiliation{INFN, Sezione di Milano, Milano, Italy}
\affiliation{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}

\author{F.~Contreras}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{F.~Convenga}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{D.~Correia dos Santos}
\affiliation{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}

\author{C.E.~Covault}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{S.~Dasso}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}

\author{K.~Daumiller}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{B.R.~Dawson}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{J.A.~Day}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{R.M.~de Almeida}
\affiliation{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}

\author{J.~de Jes\'us}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.J.~de Jong}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.R.T.~de Mello Neto}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\affiliation{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}

\author{I.~De Mitri}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.~de Oliveira}
\affiliation{Instituto Federal de Educa\c{c}\~ao, Ci\^encia e Tecnologia do Rio de Janeiro (IFRJ), Brazil}

\author{D.~de Oliveira Franco}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{F.~de Palma}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{V.~de Souza}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{E.~De Vito}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{A.~Del Popolo}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{M.~del R\'\i{}o}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{O.~Deligny}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{L.~Deval}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~di Matteo}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Dobre}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{C.~Dobrigkeit}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{J.C.~D'Olivo}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{L.M.~Domingues Mendes}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{R.C.~dos Anjos}
\affiliation{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}

\author{M.T.~Dova}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{J.~Ebr}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{R.~Engel}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{I.~Epicoco}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{M.~Erdmann}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{C.O.~Escobar}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{A.~Etchegoyen}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{H.~Falcke}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.~Farmer}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{G.~Farrar}
\affiliation{New York University, New York, NY, USA}

\author{A.C.~Fauth}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{N.~Fazzini}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{F.~Feldbusch}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Fenu}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{B.~Fick}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{J.M.~Figueira}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Filip\v{c}i\v{c}}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{T.~Fitoussi}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{T.~Fodran}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{T.~Fujii}
\altaffiliation{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{A.~Fuster}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{C.~Galea}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{C.~Galelli}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{B.~Garc\'\i{}a}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{H.~Gemmeke}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Gesualdi}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Gherghel-Lascu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{P.L.~Ghia}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{U.~Giaccari}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Giammarchi}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{J.~Glombitza}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{F.~Gobbi}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{F.~Gollan}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{G.~Golup}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{M.~G\'omez Berisso}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{P.F.~G\'omez Vitale}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{J.P.~Gongora}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{J.M.~Gonz\'alez}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{N.~Gonz\'alez}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{I.~Goos}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{D.~G\'ora}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Gorgi}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Gottowik}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{T.D.~Grubb}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{F.~Guarino}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{G.P.~Guedes}
\affiliation{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}

\author{E.~Guido}
\affiliation{INFN, Sezione di Torino, Torino, Italy}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}

\author{S.~Hahn}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Hamal}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{M.R.~Hampel}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Hansen}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{D.~Harari}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{V.M.~Harvey}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Haungs}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{T.~Hebbeker}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{D.~Heck}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{G.C.~Hill}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{C.~Hojvat}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{J.R.~H\"orandel}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{P.~Horvath}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.~Hrabovsk\'y}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{T.~Huege}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{A.~Insolia}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{P.G.~Isar}
\affiliation{Institute of Space Science, Bucharest-Magurele, Romania}

\author{P.~Janecek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.A.~Johnsen}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{J.~Jurysek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~K\"a\"ap\"a}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{K.H.~Kampert}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Keilhauer}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Khakurdikar}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{V.V.~Kizakke Covilakam}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{H.O.~Klages}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Kleifges}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{J.~Kleinfeller}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{F.~Knapp}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{N.~Kunka}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{B.L.~Lago}
\affiliation{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}

\author{N.~Langner}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{M.A.~Leigui de Oliveira}
\affiliation{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}

\author{V.~Lenok}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Letessier-Selvon}
\affiliation{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{I.~Lhenry-Yvon}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{D.~Lo Presti}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{L.~Lopes}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{R.~L\'opez}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{L.~Lu}
\affiliation{University of Wisconsin-Madison, Department of Physics and WIPAC, Madison, WI, USA}

\author{Q.~Luce}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{J.P.~Lundquist}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{A.~Machado Payeras}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{G.~Mancarella}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{D.~Mandat}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{B.C.~Manning}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{J.~Manshanden}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{P.~Mantsch}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{S.~Marafico}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{F.M.~Mariani}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{A.G.~Mariazzi}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{I.C.~Mari\c{s}}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{G.~Marsella}
\affiliation{Universit\`a di Palermo, Dipartimento di Fisica e Chimica ''E.\ Segr\`e'', Palermo, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{D.~Martello}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{S.~Martinelli}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{O.~Mart\'\i{}nez Bravo}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{M.~Mastrodicasa}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.J.~Mathes}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{J.~Matthews}
\altaffiliation{Louisiana State University, Baton Rouge, LA, USA}

\author{G.~Matthiae}
\affiliation{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{E.~Mayotte}
\affiliation{Colorado School of Mines, Golden, CO, USA}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{S.~Mayotte}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{P.O.~Mazur}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{G.~Medina-Tanco}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{D.~Melo}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Menshikov}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{S.~Michal}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.I.~Micheletti}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{L.~Miramonti}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{S.~Mollerach}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{F.~Montanet}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{L.~Morejon}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{C.~Morello}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Mostaf\'a}
\affiliation{Pennsylvania State University, University Park, PA, USA}

\author{A.L.~M\"uller}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{M.A.~Muller}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{K.~Mulrey}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{R.~Mussa}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Muzio}
\affiliation{New York University, New York, NY, USA}

\author{W.M.~Namasaka}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{A.~Nasr-Esfahani}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{L.~Nellen}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{G.~Nicora}
\affiliation{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}

\author{M.~Niculescu-Oglinzanu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{M.~Niechciol}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{D.~Nitz}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{I.~Norwood}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{D.~Nosek}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{V.~Novotny}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{L.~No\v{z}ka}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{A Nucita}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.A.~N\'u\~nez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{C.~Oliveira}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{M.~Palatka}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Pallotta}
\affiliation{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}

\author{P.~Papenbreer}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{G.~Parente}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Parra}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{J.~Pawlowsky}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{M.~Pech}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~P\c{e}kala}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{R.~Pelayo}
\affiliation{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}

\author{J.~Pe\~na-Rodriguez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{E.E.~Pereira Martins}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Perez Armand}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{C.~P\'erez Bertolli}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{L.~Perrone}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{S.~Petrera}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{C.~Petrucci}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{T.~Pierog}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Pimenta}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{V.~Pirronello}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{M.~Platino}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{B.~Pont}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Pothast}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{P.~Privitera}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{M.~Prouza}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~Puyleart}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{S.~Querchfeld}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.~Rautenberg}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{D.~Ravignani}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Reininghaus}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Ridky}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Riehn}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Risse}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{V.~Rizi}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{W.~Rodrigues de Carvalho}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{J.~Rodriguez Rojo}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{M.J.~Roncoroni}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{S.~Rossoni}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{M.~Roth}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{E.~Roulet}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{A.C.~Rovero}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}

\author{P.~Ruehl}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{A.~Saftoiu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{M.~Saharan}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{F.~Salamida}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.~Salazar}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{G.~Salina}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.D.~Sanabria Gomez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{F.~S\'anchez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{E.M.~Santos}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{E.~Santos}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Sarazin}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{R.~Sarmento}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{R.~Sato}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{P.~Savina}
\affiliation{University of Wisconsin-Madison, Department of Physics and WIPAC, Madison, WI, USA}

\author{C.M.~Sch\"afer}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{V.~Scherini}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{H.~Schieler}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Schimassek}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Schimp}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{F.~Schl\"uter}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{D.~Schmidt}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{O.~Scholten}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{H.~Schoorlemmer}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{P.~Schov\'anek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.G.~Schr\"oder}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{J.~Schulte}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{T.~Schulz}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.J.~Sciutto}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{M.~Scornavacche}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Segreto}
\affiliation{Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo (INAF), Palermo, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{S.~Sehgal}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{R.C.~Shellard}
\affiliation{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}

\author{G.~Sigl}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{G.~Silli}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{O.~Sima}
\altaffiliation{also at University of Bucharest, Physics Department, Bucharest, Romania}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{R.~Smau}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{R.~\v{S}m\'\i{}da}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{P.~Sommers}
\affiliation{Pennsylvania State University, University Park, PA, USA}

\author{J.F.~Soriano}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{R.~Squartini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.~Stadelmaier}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{D.~Stanca}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{S.~Stani\v{c}}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{J.~Stasielak}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{P.~Stassi}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{M.~Straub}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{A.~Streich}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Su\'arez-Dur\'an}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{T.~Sudholz}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{T.~Suomij\"arvi}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}

\author{A.D.~Supanitsky}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{Z.~Szadkowski}
\affiliation{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}

\author{A.~Tapia}
\affiliation{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}

\author{C.~Taricco}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{C.~Timmermans}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{O.~Tkachenko}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{P.~Tobiska}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.J.~Todero Peixoto}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{B.~Tom\'e}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{Z.~Torr\`es}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{A.~Travaini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{P.~Travnicek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Trimarelli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{M.~Tueros}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{R.~Ulrich}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Unger}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{L.~Vaclavek}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.~Vacula}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{J.F.~Vald\'es Galicia}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{L.~Valore}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{E.~Varela}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{A.~V\'asquez-Ram\'\i{}rez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{D.~Veberi\v{c}}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{C.~Ventura}
\affiliation{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}

\author{I.D.~Vergara Quispe}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{V.~Verzi}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.~Vicha}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Vink}
\affiliation{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}

\author{S.~Vorobiov}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{H.~Wahlberg}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{C.~Watanabe}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{A.A.~Watson}
\altaffiliation{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}

\author{A.~Weindl}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{L.~Wiencke}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{H.~Wilczy\'nski}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{D.~Wittkowski}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Wundheiler}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Yushkov}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{O.~Zapparrata}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{E.~Zas}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{D.~Zavrtanik}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}

\author{M.~Zavrtanik}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{L.~Zehrer}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\collaboration{0}{The Pierre Auger Collaboration}
\email{spokespersons@auger.org}

